Witness Generation for JSON Schema

JSON Schema is an important, evolving standard schema language for families of JSON documents. It is based on a complex combination of structural and Boolean assertions, and features negation and recursion. The static analysis of JSON Schema documents comprises practically relevant problems, including schema satisfiability, inclusion, and equivalence. These three problems can be reduced to witness generation: given a schema, generate an element of the schema, if it exists, and report failure otherwise. Schema satisfiability, inclusion, and equivalence have been shown to be decidable, by reduction to reachability in alternating tree automata. However, no witness generation algorithm has yet been formally described. We contribute a first, direct algorithm for JSON Schema witness generation. We study its effectiveness and efficiency, in experiments over several schema collections, including thousands of real-world schemas. Our focus is on the completeness of the language, where we only exclude the uniqueItems operator, and on the ability of the algorithm to run in a reasonable time on a large set of real-world examples, despite the exponential complexity of the underlying problem.

==> witnessgen.tex <==
% !TeX root = main_vldb.tex

\ifshort{\section{The structure of the algorithm}\label{sec:witness}}

\iflong{\subsection{The structure of the algorithm}}

Consider a recursive algorithm for witness generation.
In order to generate a witness for an {\ITO} such as
$\PReq(r:S)$, one can generate a witness $\J$ for $S$ and use it to build an object with 
a member whose name matches $r$ and whose value is $\J$. The same approach can be
followed for the other {\ITO}s.
For the Boolean operator
$S_1 \Or S_2$, one recursively generates witnesses of $S_1$ and $S_2$.

Negation and conjunction are much less direct: there is no way to generate a witness for $\Not S$ starting from a witness for $S$. Also, given a witness for $S_1$, if this is not a witness for $S_1 \And S_2$, we may
need to try infinitely many others before finding one that satisfies~$S_2$ as 
well.\iflong{\footnote{One may actually
solve the problem by ordered generation of witnesses for $S_1$ and $S_2$ and a merge-sort implementation
of intersection, but the algorithms that we explored with this approach seem far more expensive than ours.}}
We solve this problem as follows.
We first eliminate $\Not$ using not-elimination, then we bring all definitions 
of variables into DNF so that conjunctions are limited to sets of {\ITO}s that regard the
same type.
%We  then analyse these conjunctions in order to see which fresh variables
%must be defined in order to push conjunction through the {\ITO} (\emph{preparation}), and we use the 
%``{\crcombined}'' conjunctions to generate the witnesses.
We then perform a form of \emph{and-elimination} over these conjunctions,
which may require the generation of new variables (\emph{preparation}), and we finally use these 
``{\crcombined}'' conjunctions to generate the witnesses.
In this complex pipeline, \emph{preparation} is the crucial step.
%, and it is one of the main technical contributions of our work.
%
% the leaves of the syntax tree,
%and finally we make conjunction harmless by a technique that we call {\crcombination},
%which is a form of \emph{and-elimination},
%is based on the combination of all {\ITO}s having to do with the same type, and is
%presented below. After {\ITO}s and Boolean operators, we are left with recursive
%variables. We deal with them by adopting a bottom-up iterative evaluation that mimics a
%bottom-up fixpoint semantics. % defined in Section~\ref{sec:fixpoint}.
%We are now going to transform this idea into an algorithm.

%For the sake of presentation, we will first present our approach by focusing on schemas that  do not feature  $\Uni$ or $\NotUni$, and then we will present our extension to these mechanisms.
%For the sake of presentation, we will only present our approach by focusing on schemas that  do not feature  $\Uni$ or $\NotUni$. 
% will present our extension to these mechanisms.



In greater detail, our algorithm consists of the following steps.

\begin{compactenum}
\item {\textbf{ROBDD reduction}}: 
we maintain a data structure \iflong{based on ROBDD \cite{DBLP:journals/tc/Bryant86}} that allows us to discover, for any new variable that we need to introduce, 
whether it is equivalent to a variable that is already present\iflong{ in order to reuse it}; 
this is not really a ``step'' but 
something that we do any time we introduce a new variable, in order to ensure termination of the algorithm.
\item %Translation from {\jsonsch} to the core algebra, 
    \textbf{Not-completion of variables} and \textbf{not-elimination}:
    we rewrite the schema into one expressed in positive algebra\shortlong{.}{ and where each
    variable has a dual variable that corresponds to its negation.}
% and symbol reduction: we perform rewriting operations preserving semantics and ensuring that at the end of the process  $\And$ and $\Or$ are the only Boolean combinators left. %we eliminate all occurrences of $\Not$, $\Implies$, 
      %$\XOr$, so that $\And$ and $\Or$ are the only Boolean combinators left.
      %We also eliminate other symbols, moving towards the code algebra.
   \item \textbf{Stratification}: we substitute any schema argument $S$ of any {\ITO} with a fresh variable,
     whose body is $S$.
%   \item Variable normalization: we rewrite the definitions of all variables so that
%       every variable only appears as an $S$ argument of a typed operator, as in
%       $\PReq(a : x)$, and all $S$ arguments of typed operator are variables.
%        In this way, no Boolean operator has a variable as argument.
%        %This phase includes a form of not-elimination.
\item \textbf{Reduction to Canonical DNF}: 
   we transform the definition of each variable into a Canonical Disjunctive Normal Form.
  In this DNF,  every conjunction is a conjunction of {\TO}s
    that contains exactly one 
       assertion~$\Type(T)$, where~$T$ is the type of all the {\ITO}s in the conjunction.
 \item \textbf{Object and array {\crcombination}} and \textbf{variable and-comple\-tion}: we rewrite object and array 
    conjunctions 
    into a form that will allow iterative generation of witnesses. This is a form of 
    \emph{and-elimination}, where we
   precompute all variable conjunctions that we may need during the next phase,
   and associate a fresh variable to each one (\emph{and-completion}).
\item \textbf{Iterative generation}: we start from a state where the semantics of every variable is   
     unknown,
      and we repeatedly try and generate a witness for each variable, using the prepared conjunctions,
      until a fixpoint is
      reached.   %The prepared types are used to generated the witnesses.
\end{compactenum}


%Since the algebraic representation of an input schema, as well as the elimination of negation, have already been discussed, 

We now present our algorithm.
Phases (1) to (4) are presented in Section \ref{sec:firstphases}.
Phases (5) and (6) are presented in Section \ref{sec:recgen}.






\section{Towards a Canonical DNF\iflong{: ROBDDs, Not-Elimination, Stratification, GDNF Reduction, Canonicalization}}
\label{sec:firstphases}

\subsection{ROBDD reduction}\label{sec:robdd}

Two expressions built with variables
and Boolean operators are Boolean-equivalent when they can be proved equivalent using 
the laws of the Boolean algebra.
An ROBDD (Reduced Ordered Boolean Decision Diagram) is a data structure that provides the same
representation for two Boolean expressions if, and only if, they are Boolean-equivalent \cite{DBLP:journals/tc/Bryant86}.
Hence, whenever we define (or we find in the original schema) a variable $x$ whose body 
$S_x$ is a Boolean combination of variables, we perform the \emph{ROBDD reduction}:
we compute the ROBDD representation of $S_x$,
$\key{robdd}(S_x)$, and we store a 
pair $\Def{x}{\key{robdd}(S_x)}$ in the {\ROBDDT} table, unless a pair
$\Def{y}{\key{robdd}(S_y)}$ with $\key{robdd}(S_x)=\key{robdd}(S_y)$ is already present.
In this case, we substitute every occurrence of $x$ with $y$.
This data structure ensures termination of the {\crcombination} phase
(Section~\ref{sec:objprep}). 

%We have based it on the \emph{jdd} library by Arash Vahidi~\cite{jdd}.
%\ST{Suggestion: Mention jdd library in implementation/experiments section, not here.}

%Thanks to this optimization, we have exactly one variable whose body is
%$\True$, and we call it $\XTrue$, and similarly for $\XFalse$.
%For simplicity, in future examples, when the argument of a non-Boolean operator is a 
%variable whose
%body is just $\True$ or $\False$, we indicate that variable with $\True$ or $\False$,
%writing for example $\PReq(\PPP{a} :\True$) rather than $\PReq(\PPP{a} :\RRef{x})$ when the
%body of $\RRef{x}$ is $\True$.
%

\subsection{Not-elimination and not-completion}

\input{notelim.tex}


\subsection{Stratification}\label{sec:varnorm}

We say that a schema is \emph{stratified} when every schema argument of every {\ITO} is a variable,
so that 
$ \PReq{(a:\RRef{x}\And\RRef{y})}$ is not stratified
while $ \PReq{(a:\RRef{w})}$ is stratified.

\iflong{
Stratification makes it easy to build a witness for a typed group such as
$$
\TG{\Ob, \PReq(\PPP{a}:\RRef{x}), \PReq(\PPP{b}:\RRef{y})}
$$
after a witness for each involved variable has been built.}


In the \emph{stratification} phase, for every {\ITO} that has a subschema $S$ in its syntax, 
such as $\CMM{i}{j}{S}$, %$\Ex_i^j S$
when $S$ is not a variable,
we create a new variable $\Def{x}{S}$, and we substitute 
$S$ with $\RRef{x}$.  
For every variable $\Def{x}{S}$ that we define, we must also define its complement
 $\Def{not\_x}{\Not S}$, and perform not-elimination and stratification on $\Not S$. 
As specified in Section \ref{sec:robdd}, we apply ROBDD reduction to $\Def{x}{S}$
and $\Def{not\_x}{\Not S}$.



\ifshort{Stratification of a schema of size $N$ produces an equivalent sche\-ma of size $O(N)$
 \cite{attouche2022witness}.}

\iflong{
\begin{property}
Stratification transforms a schema $\Doc{S}{\E}$ into a schema $\Doc{S'}{\E'}$
such that $\semca{S}{E} = \semca{S'}{E'}$.
\end{property}

\begin{property}
Stratification transforms a schema $\Doc{S}{\E}$ into a schema $\Doc{S'}{\E'}$
such that $|\Doc{S'}{\E'}|$ is in $O(N)$, where $N = |\Doc{S}{\E}|$.
\end{property}

\begin{proof}
Assume that stratification is performed bottom up, so that  $\CMM{i}{j}{ \CMM{l}{k}{S}}$ is first transformed into 
$\CMM{i}{j}{ \CMM{l}{k}{x}}$ with  $\Def{x}{S}$ and $\Def{not\_x}{\Not S}$, and then in
$\CMM{i}{j}{y}$ with  $\Def{y}{\CMM{l}{k}{x}}$ and $\Def{not\_y}{\Not \CMM{l}{k}{x}}$. 
In this way, every $S$ that is moved
to the environment is only copied twice (once below negation), and each such operation generates two instances of $x$ and one of $\Not x$.
Hence, each node in the original tree corresponds to a constant number of nodes in the stratified tree - in the worst case, it generates three variables, one negation, and two copies of the original node. At this point we apply not-elimination,
and this step is linear as well.
\end{proof}

}













\subsection{Transformation in Canonical GDNF}\label{sec:DNF}

\subsubsection*{Guarded DNF}
A schema is in Guarded Disjunctive Normal Form (GDNF) if it 
has the shape 
$$
\Or(\And(S_{1,1},\ldots,S_{1,n_1}),\ldots,\And(S_{l,1},\ldots,S_{l,n_l}))
$$
and every $S_{i,j}$ is a {\TE}. 
Every conjunction may be trivial ($n_i = 1$), and so may be the disjunction ($l=1$).

\newcommand{\phn}{^{n}}
\newcommand{\phe}{^{G}}
\newcommand{\Ts}{{\mathcal{T}}}
\newcommand{\Sch}[2]{({#1},{#2})}

\ifshort{To transform an environment $\E$ into a corresponding one $\E\phe$ in  GDNF, we just substitute every 
variable that is not in the scope of an {\ITO}
with its body, a process that is guaranteed to terminate, thanks to the guardedness condition on 
$\E$, and we bring the result in DNF by distributivity of $\And$ and $\Or$.

Reduction to GDNF can lead to an exponential explosion, and is actually a very expensive phase, 
according to our experiments (Sect.~\ref{sec:exp}).
In greater detail, the GDNF expansion of a schema $\Doc{S}{\E}$ has size in
$O(2^{|\Doc{S}{\E}|})$, but the number of variables does not change, and this will be crucial 
in evaluating the complexity of {\crcombination} and generation.
}

\iflong{
To produce a new environment $E\phe$ in GDNF starting from a positive and stratified 
environment $E$, we first define an ordered enumeration $\Set{x_1,\ldots,x_o}$
of the variables in $\Vars(\E)$ such that when $x_i$ directly depends of $x_j$ (as defined
in Section \ref{sec:syntax}) then $j<i$. We know that such enumeration exists because 
recursion is guarded.
We now compute $E\phe(x_i)$ starting from $x_1$ and going onward, so that, when
we compute $E\phe(x_i)$, $E\phe(x_j)$ has already been computed for each $j<i$.

Let $\Ts$ denote the set of all {\TE}s that appear in $E$ as subterms of $\E(y)$ for any $y$,
 so that,
if $$\E\ \ =\ \ \Def{x}{(\TNum \And \PReq(\PPP{a}:x))\Or \Mof(3)}$$ then 
$\Ts = \Set{\TNum,\ \PReq(\PPP{a}:x),\ \Mof(3)}$.
As we will show, reduction in GDNF does not create any new typed expression, hence every 
term in GDNF corresponds to a set $DC$ (\emph{Disjunction of Conjunctions}) of subsets of $\Ts$  as follows.
$$ {\E\phe(x)} =
{\BigOr_{C \in DC_x}  \BigAnd_{S\in C}   S\ \ \ \text{where}\ \ \ \  DC_x \in \Parts(\Parts(\Ts))}$$ 



To compute this set-of-sets representation $g(E(x))$ of the GDNF of
the body $\E(x)$ of every  $x$ defined in $\E$, we apply the following rules:
$$\begin{array}{llll}
g(S) &=& \Set{\Set{S}} \qquad\qquad \mbox{\ if $S$ is a {\TE}} \\[\NL]
g(y) &=& E\phe(y)  \\[\NL]
g(S_1  \Or S_2) &=& g(S_1) \cup g(S_2)  \\[\NL]
g(S_1  \And S_2)  &=& \bigcup_{(C_1,C_2) \in g(S_1)\times g(S_2)}  (C_1\cup C_2) 
\end{array}$$

When $S$ is a typed expression, it is translated into a trivial GDNF. Each variable $y$ inside $\E(x)$ had its body
already transformed. The rule for $\Or$ is trivial, while the rule for $\And$ is Boolean algebra distributivity:
for each conjunction $\BigAnd_{S\in C_1}S$ of $S_1$ and for each conjunction $\BigAnd_{S\in C_2}$ of $S_2$, the
conjunction $\BigAnd_{S\in C_1}S \And \BigAnd_{S\in C_1}S = \BigAnd_{S\in C_1\cup C_2}S$ is inserted in the result.


%end hide


Reduction to GDNF can lead to an exponential explosion, and is actually the most expensive phase
of our algorithm, according to our measures (Sect.~\ref{sec:exp}).

\begin{property}
For a given schema $\Doc{x}{E}$, such that $n = |\Doc{x}{E}|$, the size of $\Doc{x}{E\phe}$ is in $O(2^n)$,
and it can be build in time $O(2^n)$.
\end{property}

\begin{proof}
The schema $\Doc{x}{E\phe}$ has $O(n)$ variables.
The body of each variable can be represented as a set $DC$ belonging to $\Parts(\Parts(\Ts))$
The set $\Parts(\Ts)$ has size $O(2^n)$, hence every set of sets $DC$
contain at most $O(2^n)$ sets, and each of these sets can be represented using $n$ bits.
This yields a total upper bound of $O(n)\times O(n)\times O(2^n)$ for $\Doc{x}{E\phe}$.
As for the construction time, the most expensive part is the computation of 
$\bigcup_{(C_1,C_2) \in g(S_1)\times g(S_2)}  (C_1\cup C_2)$, that may take place once
for each variable. The size of $g(S_1)\times g(S_2)$ is in $O(2^n)$, the size of $C_1$ and $C_2$
is in $O(n)$, hence this computation is in $O(2^n)$.
\end{proof}
}%end iflong





%end hide



%\iflong{\subsection{Canonicalization}}
%\ifshort{
\subsubsection*{Canonicalization}

%\GG{Remember to transform $\Not \Type{T}$}

\newcommand{\Filter}[2]{\key{filter}({#1},{#2})}

Canonicalization is a process defined along the lines of \cite{DBLP:conf/issta/HabibSHP21}.
We say that a conjunction that contains exactly one assertion $\Type(T)$ and a set of {\ITO}s of that
same type $T$ is a \emph{typed group} of type $T$; canonicalization splits every conjunct of the 
GDNF into a set of  \emph{typed groups} 
(hereafter, for brevity, we use $\TG{S_1,\ldots,S_n}$ to indicate a conjunction
$(S_1\And\ldots\And S_n$).

\ifshort{%
For example, a trivial conjunction $\{\Mof(3.5)\}$ is not a typed group, since it is missing a $\Type(T)$
assertion, and is transformed in the following disjunction of six groups:
$$
%\begin{array}{llllll}
 \{\TNum, \Mof(3.5)\}  \Or \{\TNull\}  \Or \{\TBool\} \Or \ldots
%\end{array}
$$
%After canonicalization, every conjunction denotes a set of values of the same type.
}

\iflong{%
In order to transform a conjunction $C$ of a GDNF $DC$ into a typed group, we first repeatedly apply 
the following rewriting rules, which preserve the meaning of the conjunction. In the third rule,
$\key{{\ITO}}(T')$ are the {ITO}s associated to type $T'$, which are trivially satisfied when 
in conjunction with a $\Type(T)$ with $T \neq T'$:
$$\begin{array}{llllll}
\Type(T), \Type(T) &\To & \Type(T) & \\[\NL]
\Type(T), \Type(T') &\To & \False & T \neq T' \\[\NL]
\False, S &\To & \False &\\[\NL]
\Type(T), S &\To & \Type(T) & S \in \key{{\ITO}}(T'), \ T' \neq T \\[\NL]
\end{array}
$$
The first three rules ensure that the result is either $\False$, which is then deleted from the disjunction,
or has exactly one $\Type(T)$ assertion, or has none. If it has exactly one $\Type(T)$ assertion,
then the fourth rule ensures that all the $\ITO$s refer to type $T$.
If it has no $\Type(T)$ assertion, we transform it in the following equivalent disjunction, where
$\Filter{\TG{S_1,\ldots,S_n}}{T}$ is the conjunction of those {\ITO}s in $\TG{S_1,\ldots,S_n}$ 
whose type is $T$:
%$$
%\TG{\Nl} \Or \TG{\Bo, \Filter{T'_i}{\Bo}} \Or \TG{\St, \Filter{T'_i}{\St}}\ldots
%$$
$$\begin{array}{llllll}
(\TNull) & \Or (\TBool \And \Filter{C}{\Bo}) \\
& \Or (\TStr \And  \Filter{C}{\St})\ldots
\end{array}
$$
so that every $C\in DC$ denotes a set of values of the same type.
}%end iflong

\mrevmeta{
By construction, every phase described in this section transforms a a {\JS} document into
an equivalent one.
}{M.3}

\mrevmeta{
\begin{property}[Equivalence]\label{pro:preliminarycc}
The phases of ROBDD-reduction, not-elimination, stratification, transformation 
into Canonical GDNF, transform a {\JS} document into
an equivalent one.
\end{property}
}{M.3}


\section{{\Crcombination} and \iflong{witness }generation}\label{sec:recgen}

\renewcommand{\Next}{\kw{next}}
\renewcommand{\EOV}{\kw{EOV}}
\renewcommand{\DOV}{\kw{DOV}}
\renewcommand{\AA}{A}
\newcommand{\cf}{\key{cf}}
\newcommand{\Meets}{\akey{\#}}
\renewcommand{\Meets}{\cap}
\newcommand{\JJOfD}[1]{\mathit{J}^{\mathit{#1}}}
\newcommand{\MeetsD}[1]{\cap\JJOfD{#1}}

\newcommand{\AAE}[1]{{\mathcal A}^{#1}_{\E}}
\newcommand{\AAI}{{\mathcal A}^{\Inf}_{\E}} %(\emptyset)}






\subsection{Assignments and bottom-up semantics}

\renewcommand{\Sch}{\Doc}

\ifshort{
We define an assignment $\AA$ for an environment $\E$ as a function mapping each variable of $\E$ to 
a set of {\json} values.
An assignment is sound when it maps each variable $y$ to
a subset of its semantics $\semca{y}{\E}$, which denotes the
set of {\json} values that satisfy $y$ in $\E$.}


\iflong{
Let us define an assignment $\AA$ for an environment $\E$ as a function mapping each variable of $\E$ to 
a set of {\json} values.
An assignment is sound when it maps each variable to
a subset of its semantics.
We order assignments by variable-wise inclusion.}

\newcommand{\asEval}{assignment-evaluation}

\iflong{
\begin{definition}[Assignments, Soundness, Order]
}
\ifshort{
\begin{definition}[Assignments, Soundness]
}
An assignment $\AA$ for an environment $\E$ is a function mapping each variable of $E$ to a set of {\json}
values.
%a subset of $\JJ$.
\iflong{ }
An assignment $\AA$ for $\E$ is sound iff for all $y\in \Vars(E)$, 
$\AA(\RRef{y}) \subseteq \semca{y}{\E}$.
\iflong{ 
We say that $\AA \leq \AA'$ iff $\forall y.\ \AA(y)\subseteq \AA'(y)$.}
\end{definition}

\ifshort{
Given a schema $\Sch{S}{\E}$, an assignment $\AA$ for $\E$ defines a way to evaluate
$S$ starting from $\AA$, an \emph{\asEval} $\semas{S}{\AA}$
for $S$, by applying the rules shown in Figure~\ref{tab:corealg-sem} --- we omit the trivial ones which can be found in the 
full paper.
Universal quantification on an empty set is true, and the set $\SetTo{0}$ is empty. $\semt(\Bool)$ is the set of {\json} values of type $\Bool$.

Intuitively,  $\semas{S}{\AA}$ uses the witnesses collected by
$\AA$ in order to build bigger witnesses
for $S$.
For example, if $\AA(x)=\Set{\J}$, and 
if $S={\{\TArr,\PostIte{0}{x},\CMM{1}{3}{\True}\}}$, 
 then $\semas{S}{\AA}=\Set{[\J],[\J,\J],[\J,\J,\J]}$.
}
\ifshort{% --------
\begin{figure}[tb]
\UpdateNL{0.5ex}
\[
\begin{array}{lcl}
\semas{\RRef{x}}{\AA}  &= & \AA(x) \\[\NL]
   \semas{\IBT(b)}{\AA} & = & \setst{J}{J\in\semt(\Bool) \Rightarrow  J=b }\\
%   \semas{\Pat(r)}{\AA} & = & \setst{J}{J\in\semt(\Str) \Rightarrow J \in  \rlan{r}} \\
%   \semas{\Bet_{m}^{M}}{\AA} & = & \setst{J}{ J\in\semt(\Num) \Rightarrow  m \leq J \leq M } \\
%   \semas{\XBet_{m}^{M}}{\AA} & = & \setst{J}{ J\in\semt(\Num) \Rightarrow  m < J < M } \\
%  \semas{\Mof(q)}{\AA} & = & \setst{ J}{ J\in\semt(\Num) \Rightarrow  \\
%     &&  \exists i\in\IntSet.\ J = i\cdot q} \\
\semas{\Props(\key{r} : S)  }{\AA} & = & \SetOpen\, {J} \,\mid\, J = \{(k_1:J_1),\ldots,(k_n:J_n)\} \Rightarrow  \\
     &&
   \forall i\in \SetTo{n}.\ k_i\in\rlan{r} \ \Rightarrow J_i \in \semas{S}{\AA} \,\SetClose \\
%\semas{\Req(k)}{\AA} & = & \setst{J}{J = \Set{(k_1:J_1),\ldots,(k_n:J_n)} \Rightarrow  \\
%     &&
%   \exists i\in \SetTo{n}.\ k_i = k } \\
%   \semas{\Pro_{i}^{j} }{\AA} & = & \setst{J}{J = \Set{(k_1:J_1),\ldots,(k_n:J_n)} \Rightarrow\\
%   &&    i \leq n \leq j} \\
 \semas{  \PreIte{l}{S} }{\AA} & = & \SetOpen\, {J} \,\mid\, J =  [\J_1, \ldots, \J_n ]   \Rightarrow \\
     &&
      n \geq l  \Rightarrow J_l \in   \semas{S}{\AA}  \,\SetClose  \\
 \semas{  \PostIte{i}{S} }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ]  \Rightarrow \\
     &&
     \forall j\in\SetTo{n} .\ j > i \Rightarrow J_j \in   \semas{S}{\AA} }\\
\semas{  \CMM{i}{j}{S}  }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] 
       \Rightarrow \\
     &&
      i \leq \ |\setst{l}{\J_l\in \semas{S}{\AA}}|\ \leq j }\\
%\semas{ \Uni \  }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] \Rightarrow \\
%     &&
% \forall i,j \in \SetTo{n}. \ i\neq j \ \Implies \ J_i \neq J_j}\\
% \semas{\Type(T)}{\AA}
%   & = & \semt(T)\\
 \semas{S_1 \And S_2}{\AA} & = &  \semas{S_1 }{\AA}  \cap   \semas{ S_2}{\AA} \\
 \semas{S_1 \Or S_2}{\AA} & = &  \semas{S_1 }{\AA}  \cup   \semas{ S_2}{\AA} \\
%\semas{\Not S}{\AA}  & = & \JSet \setminus \semas{S}{\AA}  \\
% \semas{\NotMof(q)}{\AA} & = & \setst{ J}{ J\in\semt(\Num) \Rightarrow \\
%     &&   \forall i\in \IntSet. \  J \neq i\cdot q} \\
 \semas{\PReq(r:S)}{\AA} & = & \setst{J}{J = \Set{(k_1:J_1),\ldots,(k_n:J_n)}   \Rightarrow \\
     &&  \exists i \in \SetTo{n} .\  k_i\in\rlan{r}) \ \And J_i \in \semas{S}{\AA} } \\
 \semas{\ContAfter{i}{S}}{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] \Rightarrow  \\
     &&   \exists l.\ l > i \ \And \J_l \in \semas{ S}{\AA} }%\\%\semas{\Doc{S}{\AA}}{}  & = & \semas{S}{\AA}  \\
%\semas{\Doc{S}{\AA}}{}  & = & \semas{S}{\AA}  \\
 \end{array}
\]
\RestoreNL
\caption{Rules for assignment evaluation.}
\label{tab:corealg-sem}
\end{figure}
}%end ifshort

%\ST{Pls. cross-check caption for Figure~\ref{tab:corealg-sem}.}

\iflong{
Given a schema $\Sch{S}{\E}$, an assignment $\AA$ for $\E$ defines an \emph{\asEval}
for $S$ by applying the rules in Figure \ref{tab:corealg-set}, 
which are the same rules that define environment-based
semantics $\semca{S}{\E}$, with the only difference that a variable $\RRef{x}$ is not interpreted
by interpreting the schema $\E(x)$, but directly as the set of values $\AA(x)$
(we always assume that every schema $\Sch{S}{\E}$ is closed and guarded).


For all schemas  not containing subschemas, such as $\IBT(b)$, we just define
$\semas{\IBT(b)}{\AA} = \semca{\IBT(b)}{\E}$, and neither $\AA$ nor $\E$ play any role in the definition
\begin{figure}[ht]

\[
\begin{array}{lcl}
\semas{\RRef{x}}{\AA}  &= & \AA(x) \\[\NL]
   \semas{\IBT(b)}{\AA} & = & \setst{J}{J\in\semt(\Bool) \Rightarrow  J=b }\\[\NL]  
  \semas{\Props(\key{r} : S)}{\AA} & = & \setst{J}{J = \{(k_1:J_1),\ldots,(k_n:J_n)\} \Rightarrow  \\
     &&
   \forall i\in \SetTo{n}.\ k_i\in\rlan{r} \ \Rightarrow J_i \in \semas{S}{\AA} } \\[\NL]
\iflong{
\semas{\PreIte{l}{S} }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] \Rightarrow  \\
     &&
          n \geq l \Rightarrow J_l \in   \semas{  S }{\AA} }\\[\NL]        
\semas{  \CMM{i}{j}{S}  }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] 
       \Rightarrow \\
     &&
      i \leq \ |\setst{l}{\J_l\in \semas{S}{\AA}}|\ \leq j }\\[\NL]
}%end iflong
%\semas{ \Uni \  }{\AA} & = & \setst{J}{ J =  [\J_1, \ldots, \J_n ] \Rightarrow \\
%     &&
% \forall i,j \in \SetTo{n}. \ i\neq j \ \Implies \ J_i \neq J_j}\\
 \semas{S_1 \And S_2}{\AA} & = &  \semas{S_1 }{\AA}  \cap   \semas{ S_2}{\AA} \\[\NL]
\iflong{
 \semas{S_1 \Or S_2}{\AA} & = &  \semas{S_1 }{\AA}  \cup   \semas{ S_2}{\AA} \\[\NL]
}
 \ldots
 \end{array}
\]
\caption{Rules for {\asEval}.}
\label{tab:corealg-set}
\end{figure}

For schemas in the positive algebra, iterated
{\asEval} yields an alternative notion of semantics, as follows.
}%end iflong


\ifshort{
Hence, the repeated application of these rules, 
used to define increasingly bigger witnesses for a set of variables starting from an empty assignment  $\AAE{0}$, 
defines a sequence of assignments $\AAE{i}$, whose limit $\AAI$ defines a bottom-up semantics for
{\jsonsch}.


\begin{definition}[$\AAE{i}$, $\AAI$]
For a given positive environment $\E$, the sequence of assignments $\AAE{i}$ is defined 
as\iflong{ follows}:
$$
\begin{array}{llllllllll}
% & \AAE{0} &=& \lambda y. \emptyset \\[\NL]
% & \AAE{i+1} &=& \lambda y. \semas{\E(y)}{\AAE{i}} \\
\forall y\in\Vars(\E):&  &\AAE{0}(y) = \emptyset 
&&
 & \AAE{i+1}(y) =  \semas{\E(y)}{\AAE{i}} \\
\end{array}
$$

The assignment $\AAI$ is defined as $\bigcup_{i \in \Nat}\AAE{i}$.
\end{definition}

}%end ifshort




\iflong{
\begin{definition}
For a given positive environment ${\E}$, the corresponding assignment transformation $T_{\E}(\_)$ is the function from assignments to assignments defined as follows:
$$\begin{array}{llll}
\forall y\in\Vars(\E).\ T_{\E}(\AA)(y) = \semas{\E(y)}{\AA}
\end{array}$$
\end{definition}


Intuitively, if $\AA$ collects witnesses for the variables in $\E$,
then $T_{\E}(\AA)$ uses $\E$ in order to build new witnesses
starting from those in $\AA$.
For example, if $\E$ contains $\Def{y}{\{\TArr,\PostIte{0}{x},\CMM{1}{3}{\True}\}}$, 
if $\AA(x)=\Set{\J}$, then $T_{\E}(\AA)(y)=\Set{[\J],[\J,\J],[\J,\J,\J]}$.


For any positive environment $\E$, the corresponding assignment transformation is monotone in $\AA$, by positivity
of $\E$, hence $T_{\E}$ has a minimal fixpoint, 
that is the limit $\AAI$ of the sequence $\AAE{i}$ defined accordingly
to Tarski theorem, starting from the empty assignment and then reapplying $T_{\E}$.

\begin{definition}[$\AAE{i}$, $\AAI$]
For a given positive environment $\E$, the sequence of assignments $\AAE{i}$ is defined 
as\iflong{ follows}:
$$
\begin{array}{llllllllll}
% & \AAE{0} &=& \lambda y. \emptyset \\[\NL]
% & \AAE{i+1} &=& \lambda y. \semas{\E(y)}{\AAE{i}} \\
& \forall y\in\Vars(\E).\ \AAE{0}(y) = \emptyset 
\shortlong{&&}{\\[\NL]}
 & \AAE{i+1} = T_{\E}(\AAE{i}) \\
\end{array}
$$

The assignment $\AAI$ is defined as $\bigcup_{i \in \Nat}\AAE{i}$.
\end{definition}

\begin{property}
For any positive ${\E}$, the assignment $\AAI$ is the minimal fixpoint
of the assignment transformation $T_{\E}$.
\end{property}
}

\ifshort{
The function $\semca{S}{\E}$ described in the full paper \cite{attouche2022witness} corresponds to the official semantics,
since we expand
each variable $x$ to its definition $\E(x)$ and we treat negation as complement.
In the full paper, we show that on positive schemas, the bottom-up interpretation
$\semas{S}{\AAI}$ corresponds to the top-down interpretation $\semca{S}{\E}$.
}

\iflong{
In Section \ref{sec:semantics}, we adopted the official top-down semantics for {\json} schema in order to follow the standard and
because it also applies to negative operators. However, on positive schemas, the top-down semantics and the
bottom-up fixpoint coincide.

\begin{property}
For any positive schema $\Sch{S}{\E}$, %for any $y$ defined in $\E$, 
the following equality holds:
$$
\semca{S}{\E} = \semas{S}{\AAI}
$$
\end{property}
}

\iflong{
\begin{proofsketch}
We prove, by induction on $i$ and, when $i$ is equal, on $S$, that for all $i$, and for any positive 
assertion $S$ that is closed 
wrt $\E$, the following holds:
$$\semcai{S}{\E} = \semas {S}{\AAE{i}}
$$
For the inductive step $i+1$, if $S$ is an operator that contains no schema subterm, the equality
$$\semcapar{S}{\E}{i+1} = \semas {S}{\AAE{i+1}}
$$ is immediate.
If $S$ is a variable, we have, by definition,
$\semcapar{y}{\E}{i+1}=\semcapar{\E(y)}{\E}{i}$
and
$\semas{y}{\AAE{i+1}} = (\AAE{i+1})(y) = \semas{\E(y)}{\AAE{i}}$;
we can conclude since
$\semcapar{\E(y)}{\E}{i} = \semas{\E(y)}{\AAE{i}}$ holds by induction on $i$.
For  $S=S_1 \And S_2$ we reason by induction on $S$ as follows:  
$$\begin{array}{llll}
\semcapar{S_1 \And S_2}{\E}{i+1}
 = \semcapar{S_1}{\E}{i+1}\cap \semcapar{ S_2}{\E}{i+1}\\[\NL]
 = \semas{S_1}{\AAE{i+1}}\cap\semas{S_2}{\AAE{i+1}}
 =\semas{S_1\And S_2}{\AAE{i+1}}
\end{array}$$
For all other operators we reason in the same way.

Finally, the base case $i = 0$. 
When $S=x$, then both $\semcapar{x}{\E}{0}$ and $\semas{x}{\AAE{0}}$ are the empty set.
In all other cases, we reason as in case $i>0$.



Now, since $\semcap{S}{\E}$ coincides with $\semas{S}{\AAE{p}}$ for any $p$, 
then $\semcap{S}{\E}$ is a succession of sets that grows with $p$, 
hence $\bigcap_{p \geq i}\semcapar{S}{\E}{p} = \semas{S}{\AAE{i}}$,
hence $\bigcup_{i\in N}\bigcap_{p \geq i}\semcapar{S}{\E}{p}
= \bigcup_{i\in\Nat} \semas{S}{\AAE{i}}
= \semas{S}{\AAI}$.

\end{proofsketch}
}

Any {\json} value $\J$ has a \emph{depth} $\Dep(\J)$, that is the number of levels of its tree
representation, formally defined as follows.

\begin{definition}[Depth $\Dep(\J)$, $\JJOfD{\key{dep}}$]
The depth of a {\json} value $\J$, $\Dep(\J)$, is defined as follows, where $\max(\Set{\ })$ 
is defined to be 0:
$$\begin{array}{lllllllll}
\mbox{$\J$ belongs to a base type}: & \Dep(\J) = 1  \\[\NL]
\J = [\J_1,\ldots,\J_n]:                     & \Dep(\J) = 1 + \max(\Set{\Dep(\J_1),\ldots,\Dep(\J_n)}) \\[\NL]
\J = \{ \ \key{a_1}: \J_1,\ldots, \key{a_n}: \J_n\ \}:      & \Dep(\J) = 1 + \max(\Set{\Dep(\J_1),\ldots,\Dep(\J_n)}) \\[\NL]
\end{array}$$

$\JJOfD{\key{dep}}$ is the set of all {\json} values $\J$ with $\Dep(\J)\leq dep$.

\end{definition}

The assignment $\AAE{i}$ includes all witnesses of depth $i$:
%$for any $\J\in \semca{y}{\E}$, it can be proved that $\J\in \AAE{\Dep(\J)}(y)$.
for any depth $i$, it can be proved that $(\semca{y}{\E}\MeetsD{i})\subseteq \AAE{i}(y)$.
%\ifshort{This almost immediately implies that $\semcai{S}{\E}=\semas{S}{\AAE{i}}$.}



\iflong{%
Bottom-up semantics is the basis of bottom-up witness generation: we will compute a witness for $\Sch{S}{\E}$
by approximating the sequence $\AAE{i}$.
}

\subsection{Bottom-up iterative witness generation}\label{sec:bottomup}
\ifshort{\label{sec:implementation}}

\newcommand{\Gen}{\ensuremath{\mathit{Gen}}}

Since $\Sch{S}{\E}$ is equivalent to $\Sch{x}{\Def{x}{S},\E}$, we will discuss here, for
simplicity, generation for the $\Sch{x}{\E}$ case.

Our algorithm for bottom-up iterative witness generation for a schema $\Sch{x}{\E}$
produces a sequence of finite assignments $\AA^i$, each approximating the assignment $\AAE{i}$,
until we reach either a witness for $x$ or an ``unsatisfiability fixpoint'', 
which is a notion that we will introduce shortly.

$\AA^i$ is defined as follows: $\AA^0=\AAE{0}$;
for each $y\in\Vars(\E)$, we let 
$\AA^{i+1}(y)=\Gen(\E(y),\AA^i)$, where
\Gen\ is an algorithm that computes a finite subset of $\semas{\E(y)}{\AA^{i}}$.
 \Gen\ is defined later, but any algorithm can be used provided it is 
\emph{sound} and \emph{generative}, as defined below. 

We first 
introduce a notion of \emph{$i$-witnessed assignment} $\AA$:
if a variable $y$ has a witness $\J$ with $\Dep(\J)\leq i$, then $y$ has a witness 
in $\AA$.
%which captures a fundamental 
%property of $\AAE{i}$ that is also enjoyed by its approximation
%$\AA^{i}$.

\begin{definition}[$i$-witnessed]
For a given environment $\E$, and an
assignment $\AA$ for $\E$, we say that $\AA$ is $i$-witnessed if:
$$\forall y\in\Vars(\E). \ (\semca{y}{\E}\MeetsD{i})\neq \emptyset\ 
\Implies\ \AA(y)\neq\emptyset
$$
%$$\forall y\in\Vars(\E). \ \AAE{i}(y)\neq \emptyset\ 
%\Implies\ \AA(y)\neq\emptyset
%$$
\end{definition}

{Generativity of $g$ means, informally, that, whenever 
$\AA$ is $i$-witnessed, then the assignment computed using
$g$ is ($i$+1)-witnessed.}
%, and both properties are crucial.

Hereafter, we say that a triple $(S,\E,\AA)$ is coherent if $\E$ is guarded and closing
for $S$, and if $\Vars(\E)=\Vars(\AA)$.

\begin{definition}[Soundness of $g$]
A function
$g(\_,\_)$ mapping each pair assertion-assignment to a set of {\json} values is \emph{sound}
iff, for every coherent $(S,\E,\AA)$,
if $\AA$ is sound for ${\E}$, then $g(S,\AA)\subseteq \semca{S}{\E}$.
%A function
%$f(\_,\_)$ mapping each pair schema-assignment to a set of {\json} values is \emph{sound}
%iff whenever $\AA$ is sound for $\Sch{S}{\E}$, then $f(\Sch{S}{\E},\AA)\subseteq \semas{S}{\AA}$.
\end{definition}

\begin{definition}[Generativity of $g$]\label{def:gen}
A function
$g(\_,\_)$ mapping each pair assertion-assignment to a set of {\json} values is \emph{generative}
for an assertion  $S$ iff for any $\E$ and $\AA$ such that $(S,E,A)$ is coherent:
\begin{compactenum}
\item if $(\semca{S}{\E}\MeetsD{1}) \neq \emptyset$, then $g(S,\AA) \neq \emptyset$;
\item for any $i\geq 1$, if $\AA$ is $i$-witnessed, and if
   $(\semca{S}{\E}\MeetsD{i+1}) \neq \emptyset$,   then $g(S,\AA) \neq \emptyset$.
   % of depth $d+1$.
\end{compactenum}
$g$ is generative for $\E$ if it is generative for $\E(y)$ for each variable $y\in \Vars(\E)$.
\end{definition}

\iflong{
Soundness of \Gen\ inductively implies that every assignment in every $\AA^i$ is sound.
Generativity implies that each $\AA_i$ computed by the $i$-th pass of the algorithm is
$i$-witnessed, so that, if a variable has a witness $\J$ of depth $d$, then
$\AA^{i}\neq \emptyset$ for every $i \geq d$.}

We can now define our bottom-up algorithm %, based on the idea we just described, 
as follows.
\RestyleAlgo{ruled}
\begin{algorithm}\label{alg:bottomup}
\footnotesize
\caption{Bottom up witness generation}
\SetKwProg{Fn}{}{}{end}
\SetKw{kwWhere}{where}
\SetKwFunction{BotUp}{BottomUpGenerate}
\SetKwFunction{Prepare}{Prepare}
\SetKwFunction{Eval}{Eval}
\SetKwFunction{Gen}{Gen}

\Fn{\BotUp{x,E}}{ 
  \Prepare(E)\;
  $\forall y.\ A[y] := \text{nextA}[y] := \emptyset$ \; 
  \While{A[x] == $\emptyset$}{  
    \For{y in vars(E) \kwWhere A[y] == $\emptyset$}{
        $\text{nextA}[y] :=  \Gen{\E(y),A}\;$}
     \lIf{($\forall y.\ $nextA[y] == A[y])} {\Return (unsatisfiable)} 
     \Else{$\forall y.\ A[y] := \text{nextA}[y]$\;}
   } 
   \Return ($A[x]$)\;
} 
\end{algorithm}

\emph{Prepare(E)} rewrites $\E$ and prepares all the extra variables needed for generation,
as explained later.
Then, we initialize $\AA^0$ as the empty assignment $\lambda y.\ \emptyset$.
We repeatedly execute a pass that
sets $\AA^{i}(y) =  \Gen(\E(y),\AA^{i-1})$ for any $y$ such 
that  $\AA^{i-1}(y) =\emptyset$ ---
we call it ``pass $i$''.
We say that a pass~$i$ is \emph{useful} if there exists $y$ such that 
$\AA^{i}(y)\neq\emptyset$ while $\AA^{i-1}(y)=\emptyset$, and we say that pass
$i$ was \emph{useless} otherwise.
Before each pass $i$, if $\semas{x}{\AA^{i-1}}\neq\emptyset$, then the algorithm stops with success. 
After pass $i$, if the pass was useless, the algorithm stops with ``unsatisfiable''.







\iflong{%
We can now prove that this algorithm is correct and complete, as follows.
}

\begin{property}[Correctness and completeness]\leavevmode\label{pro:coandco}
%\mbox{\ \ }\\
If \Gen\ is sound and is generative for $\E$ after preparation, then Algorithm 1 enjoys the following properties.
\begin{compactenum}
\item If the algorithm terminates with success after step $i$, then 
%$\semas{x}{\AA^i}$
$A^i(x)$ is not empty and
is a subset of $\semca{x}{\E}$.
\item If the algorithm terminates with ``unsatisfiable'', then $\semca{x}{\E} = \emptyset$.
\item The algorithm terminates after at most $|\Vars(\E)|+1$ passes.
\end{compactenum}
\end{property} 

\ifshort{
\bcolormeta
\begin{proof}
\mrevmeta{Proof hint, for full proof see \cite{attouche2022witness}.
Property (1) is immediate.
}{M.3}
For (2), we first prove the following property: if the algorithm terminates 
with ``unsatisfiable'' after step $j$, then, for every variable $y$:
$\AA^{j}(y)=\emptyset \ \Implies\ \semca{y}{\E}= \emptyset.$
Assume, towards a contradiction, that there is a non empty set of variables $Y$ such that
$y\in Y\ \Implies\ (\AA^{j}(y)=\emptyset  \ \And\   \semca{y}{\E}\neq\emptyset).$
Let $d$ be the minimum depth of $\bigcup_{y\in Y}\semca{y}{\E}$, and let
$w$ be a variable in $Y$ and such that $d$ is the minimum depth of the
values in $\semca{w}{\E}$.
Minimality of $d$ implies that every variable $z$ with a value in $\semca{z}{\E}$ 
whose depth is less than
$d-1$ has a witness in $\AA^{j}$, hence, since the step $j$ was useless,
every such $z$ has a witness in $\AA^{j-1}$,
hence  $\AA^{j-1}$ is $(d-1)$-witnessed, hence, by generativity, $w$ should have a witness 
generated during step $j$, which contradicts the hypothesis.

If the algorithm terminates with ``unsatisfiable'', this means that $\semas{x}{\AA^{j-1}}=\emptyset$,
hence $\semas{x}{\AA^{j}}=\emptyset$ since the step $j$ was useless, hence $\semca{x}{\E}=\emptyset$,
since we proved that 
$\AA^{j}(y)=\emptyset \Implies \semca{y}{\E}=\emptyset.$

Property (3) holds since at every useful pass the number of variables such that $\AA^i(y)\neq\emptyset$
diminishes by at least 1.
\end{proof}
\ecolormeta
}

\iflong{
\begin{proof}
Property (1) is immediate:
by induction and by soundness of $\Gen$, we have that 
${\AA^i}$ is sound for any $i$, that is,
$\semas{S}{\AA^i} \subseteq \semca{S}{\E}$.



For (2), we first prove the following property: if the algorithm terminates 
with ``unsatisfiable'' after step $j$, then, for every variable $y$:
$$\AA^{j}(y)=\emptyset \ \Implies\ \semca{y}{\E}= \emptyset.$$
Assume, towards a contradiction, that there is a non empty set of variables $Y$ such that
$$y\in Y\ \Implies\ (\AA^{j}(y)=\emptyset  \ \And\   \semca{y}{\E}\neq\emptyset).$$
Let $d$ be the minimum depth of $\bigcup_{y\in Y}\semca{y}{\E}$, and let
$w$ be a variable in $Y$ and such that $d$ is the minimum depth of the
values in $\semca{w}{\E}$.
Minimality of $d$ implies that every variable $z$ with a value in $\semca{z}{\E}$ 
whose depth is less than
$d-1$ has a witness in $\AA^{j}$, hence, since the step $j$ was useless,
every such $z$ has a witness in $\AA^{j-1}$,
hence  $\AA^{j-1}$ is $(d-1)$-witnessed, hence, by generativity, $w$ should have a witness 
generated during step $j$, which contradicts the hypothesis.

If the algorithm terminates with ``unsatisfiable'', this means that $\semas{x}{\AA^{j-1}}=\emptyset$,
hence $\semas{x}{\AA^{j}}=\emptyset$ since the step $j$ was useless, hence $\semca{x}{\E}=\emptyset$,
since we proved that 
$$\AA^{j}(y)=\emptyset \Implies \semca{y}{\E}=\emptyset.$$

Property (3) is immediate: at every useful pass the number of variables such that $\AA^i(y)\neq\emptyset$
diminishes by at least 1, hence we can have at most $|\Vars(\E)|$ useful passes plus one useless pass.
\end{proof}
}

Not every schema $S$ has a sound function that is generative for it.
Definition \ref{def:gen} (2) implies that \Gen\ is able to verify whether 
$(\semca{S}{\E}\MeetsD{i+1})\neq \emptyset$
only knowing \emph{one} arbitrary value of  $\semca{x}{\E}$ for any variable such that
$(\semca{x}{\E}\MeetsD{i})\neq \emptyset$.
This requires a certain degree of ``independence'' of the different assertions inside $S$. 
%Consider for example an array group 
%$$S=\TG{\TArr, \CMM{2}{2}{\True},  \CMM{1}{\Inf}{\RRef{x}}, \CMM{1}{\Inf}{\RRef{y}} }$$
%with
%$\E = \Def{x}{\True}, \Def{y}{\True}$. %; any $[\J_1, \J_2]$ array is a depth-2 witness for $S$ in $\E$.
%Consider   $\AA^1$ with $\AA^1(x)=\Set{12}$ and $\AA^1(y)=\Set{34}$:
%a \Gen\ function can compute a witness $ [ 12, 34 ] $ for $S$ starting from $\AA$.
Consider for example an array group
$$S=\TG{\TArr, \CMM{1}{1}{\True},  \CMM{1}{\Inf}{\RRef{x}}, \CMM{1}{\Inf}{\RRef{y}} }$$
Let $\E = \Def{x}{\True}, \Def{y}{\True}$. %; in this case, any $[\J_1]$ array is a depth-2 witness for $S$ in $\E$.
The group is 2-witnessed in $\E$ by any array $[\J]$.
Hence, a function generative for $S$ must be able to generate a witness starting from any $1$-witnessed assignment,
such as $\AA(x)=\Set{12}$ and $\AA(y)=\Set{34}$, but this is impossible, since the assignment does not
provide any value that satisfies both $x$ and $y$, and a sound function can not attribute to $x$ or $y$ any
value that is not included in the assignment.
If we want to generate a witness for $S$ with our approach, we must first rewrite $S$ in a form that makes
the interaction of the different assertions explicit, for example by adding to $\E$ a fresh variable
$z$ equivalent to $x\And y$ and by rewriting $S$ as
$\TG{\TArr, \CMM{1}{1}{\True},  \CMM{1}{\Inf}{\RRef{z}} }$.


For this reason, our bottom-up approach requires a preliminary \emph{\crcombination} phase where 
we make every interaction between assertions explicit, at the price of introducing new variables,in order to 
 remain with interaction-free schemas where the ability to build a witness for $S$ from witnesses for its free variables
 only depends on which of these variables have a witness, but not the specific witness provided for them.


%\iflong


\iflong{%
We can finally describe the phases of {\crcombination} and generation for all typed groups.
}

\ifshort{%
We finally describe the phases of {\crcombination} and generation for object groups, corresponding
respectively to the functions \emph{Prepare} and \emph{Gen} of Algorithm 1. %\ref{alg:bottomup}.
For reasons of space we will only sketch the same phases for array groups. 
Generation for strings and numbers is much simpler
and is described in the full paper \cite{attouche2022witness}.
}

\input{objectprep.tex}


\ifshort{%
\subsection{Array group {\crcombination} and generation}\label{subsec:arraygrprep}

In theory, arrays and objects are almost identical, since they are both finite mappings from labels to
values. However, arrays introduce additional issues:
\begin{compactenum}
\item Arrays have a domain downward closure constraint, that specifies that, when a value is associated to a label $n+1$, then a value is associated to $n$ as well, for every $n \geq 1$;% objects do not have anything similar.
\item The $\CMM{i}{j}{\RRef{x}}$ operator specifies an upper bound, and requires counting,
while $\PReq(\key{a}:\RRef{x})$ only specifies the existence of at least one member matching $a$ with 
schema $\RRef{x}$, with no upper bound and no counting ability.
\end{compactenum}

Our approach for array preparation and generation is still based on \emph{lazy and-completion}, guided by 
a notion of \emph{choices}, but the nature of array choices, and the strategy that we use in order to explore
them, are quite different. For more details, see \cite{attouche2022witness}.
}

\iflong
{%
\subsection{Array group {\crcombination} and generation}\label{subsec:arraygrprep}

\subsubsection{Constraints and requirements} 

As with objects, we say that an assertion $S=\ContAfter{i}{\RRef{x}}$  or $S=\CMM{i}{\Inf}{\RRef{x}}$ with $i>0$ is a
\emph{requirement}, since it is not satisfied by $[\,]$ and, if $\J^+$ extends $\J$, then 
$\J\in\semca{S}{\E}\Implies\J^+\in\semca{S}{\E}$.

We say that an assertion $S=\PreIte{l}{\RRef{x}}$, $S=\PostIte{i}{\RRef{x}}$,  
or $S=\CMM{0}{j}{\RRef{x}}$ is a
\emph{constraint}, since it is satisfied by $[\,]$ and  if $\J^+$ extends $\J$, then 
$\J^+\in\semca{S}{\E}\Implies\J\in\semca{S}{\E}$.

An assertion $S=\CMM{i}{j}{\RRef{x}}$ with $i\neq 0$ and $j\neq \Inf$ combines a requirement and a constraint.
%As a consequence, a possible algorithm to build an object is: start from the empty object, add one field
%at a time until all requirements are satisfied, but, whenever you add a field to satify \emph{some} requirements,
%verify that \emph{all} constraints are satisfied by that field.

\subsubsection{Array group {\crcombination}}


\renewcommand{\IJ}[2]{[{#1},{#2}]}
\newcommand{\Inter}{\key{In}}
\newcommand{\HL}{\key{HL}}
\newcommand{\hel}{head-length}


An array group is a set of assertions with the following shape:
$$\{\ \TArr, IP, AP, KP\ \}
$$
Here, $IP$ is a set of \emph{item} constraints $\PreIte{l}{\RRef{x}}$ and $\PostIte{i}{\RRef{x}}$,
$AP$ is a set of \emph{contains-after} requirements with shape $\ContAfter{l}{\RRef{x}}$,
$KP$ is a set of \emph{counting} assertions $\CMM{i}{j}{\RRef{x}}$, where every assertions combines
a requirement $\CMM{i}{\Inf}{\RRef{x}}$ and a constraint $\CMM{0}{j}{\RRef{x}}$.%
\footnote{For the sake of simplicity, in our formal treatment we do not distinguish
$\CMM{i}{j}{\XTrue}$ from the other counting assertions, where $\XTrue$ here indicates the variable whose body is $\True$,
although in the implementation we actually exploit its special properties for efficiency reasons.}

In theory, arrays and objects are almost identical, since they are both finite mappings from labels to
values, but arrays have some extra issues:
\begin{compactenum}
\item Arrays have a domain downward closure constraint, that specifies that, when a value is associated to a label $n+1$, then a value is associated to $n$ as well, for every $n \geq 1$; objects do not have anything similar.
\item The $\CMM{i}{j}{\RRef{x}}$ operator specifies an upper bound, and requires counting,
while $\PReq(\key{a}:\RRef{x})$ only specifies the existence of at least one member matching $a$ with 
schema $\RRef{x}$, with no upper bound and no counting ability.
\end{compactenum}

Consider for example the following array group.
$$ \{\ \TArr, \PreIte{2}{\RRef{x}}, \ContAfter{0}{\RRef{y}}, \CMM{1}{1}{\RRef{z}}, 
\CMM{2}{2}{\XTrue} \}
$$

It describes an array of exactly two elements. The one at position 2 must satisfy $\RRef{x}$.
At least one of the two elements must satisfy $\RRef{y}$.
One, but only one, of the two elements must satisfy $\RRef{z}$.

Let us say that an array has shape $[S_1,\ldots,S_k]$ if it contains exactly $k$ items
$[\J_1,\ldots,\J_k]$, and if each item $\J_i$ satisfies $S_i$.
Then, the group above is satisfied by arrays with one of the following four shapes:
$$\begin{array}{lllllllllllll}
\ [\ \RRef{y} \And \RRef{z},\ &\RRef{x} \And \NR{z}\ ], &
\ [\ \RRef{y} \And \NR{z} ,\ &\RRef{x} \And \RRef{z}\ ],  \\
\ [\ \RRef{z} ,\ &\RRef{x} \And \RRef{y} \And \NR{z}\ ], &
\ [\ \NR{z}, \ &\RRef{x} \And \RRef{y} \And \RRef{z}\ ] 
\end{array}$$

We recognize the two problems that we have seen with objects: interaction between constraints and requirements,
resulting in conjunctions of $\RRef{x}$ with other variables in position 2,
and the possibility of one element to satisfy two requirements, resulting in $\RRef{y} \And \RRef{z}$
conjunctions, but we have the extra problem of the upper bound, that results in the presence of 
the dual variable $\NR{z}$ in some positions.

Hence, our algorithm to {\crcombine} arrays and to generate the corresponding witnesses is somehow different
from that of objects, although similar in spirit. It obviously differs in the presence of dual variables like $\NR{z}$, motivated
by upper bounds, but also differs in the strategy that we use to explore the space of witnesses. Instead of starting
the exploration from the requirements, hence from the ``first choices'', here we are guided by the 
domain closure constraint, hence we start the exploration from the first position of the array.

We need to define some terminology.
We first define a notion of head-length for an array group $S$ (Definition \ref{def:head}):
intuitively, when the head-length of $S$ is $h$, then, for any witness $\J$ of $S$, if the elements of $J$ from position $h+1$ onwards --- which constitute the \emph{tail} of $\J$ --- are permuted, then 
$\J$ is still a witness; the elements in positions $1$ to $h$ constitute the \emph{head}, and their
position may matter.
For example, an array group $\{\TArr, \PreIte{3}{x}\}$ has head-length 3.
%a head-length of
%$n$ means that if an array $\J_1,\ldots,\J_l$ satisfies the group, then the array obtained by
%exchanging two elements $\J_i$ and $\J_j$ with $i>n$ and $j>n$ still satisfies the group.
The head-length $n$ may be $0$, and actually this is the most common {\hel} that we
encounter in practice.
The interval of an assertion $\Inter(S)$ is the interval of positions of the array 
that the assertion describes,
which may belong to the head of the group, to the tail, or may cross both. 

\begin{definition}[$\IJ{i}{j}$, $\HL(S)$, $\Inter(S)$]\label{def:head}
$\IJ{i}{j}$, with $i\in\Nat, j\in\Nat^{\Inf}$, denotes the interval between $i$ and $j$, which is infinite when $j=\Inf$, and is empty
when $i>j$.
The head-length $\HL(S)$ and the interval $\Inter(S)$ of an array {\ITO} $S$,
and of an array group, %$S = \{ \TArr, IP, AP, KP \}$, 
are  defined as follows:
$$\begin{array}{llllllll}
\IJ{i}{j} & = & \setst{l}{ l\in\Nat,\  i \leq  l \leq j} \\[\NL]
\HL(\PreIte{l}{S}) & = & l & \\[\NL]
\HL(\PostIte{i}{S}) & = & i & \\[\NL]
\HL(\ContAfter{l}{S}) & = & l \\[\NL]
\HL(\CMM{i}{j}{S}) & = & 0 \\[\NL]
\HL((\{ \TArr, IP, AP, KP \}) & = & \max_{S\in IP\cup AP}(\HL(S))  \\[\NL]
\Inter(\PreIte{l}{S}) & = & \IJ{l}{l} & \\[\NL]
\Inter(\PostIte{i}{S}) & = & \IJ{i+1}{\Inf} & \\[\NL]
\Inter(\ContAfter{l}{S}) & = & \IJ{l+1}{\Inf} \\[\NL]
\Inter(\CMM{i}{j}{S}) & = & \IJ{1}{\Inf} \\[\NL]
\end{array}
$$
\end{definition}

\begin{property}[Irrelevance of tail position]
If $S$ is an array typed group, $J=[\J_1,\ldots,\J_n]\in\semca{S}{\E}$, 
for all $i, j$ with
 $HL(S) < i \leq j \leq n$, if $\J'$ is obtained from $\J$
by exchanging $\J_i$ with $\J_j$, then $J'\in\semca{S}{\E}$.
\end{property}

In order to define a choice we need a last definition: for a set of assertions 
$\mathcal{S}$, we define its restriction to $\IJ{i}{j}$, denoted by
$\mathcal{S} \Meets \IJ{i}{j}$, as the subset of $\mathcal{S}$ containing the
assertions whose interval intersects $\IJ{i}{j}$.

\begin{definition}[$\mathcal{S} \Meets \IJ{i}{j}$]
$$\mathcal{S} \Meets \IJ{i}{j} = \setst{S}{S\in \mathcal{S}, \ (\IJ{i}{j} \cap \Inter(S)) \neq \emptyset}$$
\end{definition}



Now, we define a choice for an array group $IP$, $AP$, $KP$ with $h=\HL(IP\cup AP)$,
as a quintuple $(\IJ{i}{j},IP',AP',KP^{+},KP^{-})$ %with $1 \leq i \leq h+1$ and 
where:
\begin{compactenum}
\item either $i=j \leq h$ or $i=h+1$ and $j=\Inf$, hence a choice describes either
     a single element $\IJ{i}{i}$ in the head of the array group, or an element in the tail
     interval $\IJ{h+1}{\Inf}$;
\item $IP'$ is equal to $IP \Meets \IJ{i}{j}$;
% (that is, either 
   %   $IP \Meets \IJ{i}{i}$ with $i\leq h$, or $IP \Meets \IJ{h+1}{\Inf}$);
\item $AP'$ is a subset of $AP \Meets \IJ{i}{j}$;
\item $KP^{+}$ is a subset of $KP$;
\item $KP^{-}$ is a subset of $KP \setminus KP^{+}$.
\end{compactenum}

Hence, for each interval $\IJ{i}{j}$, the element $IP'$ is fixed, but we may still have many choices for 
$AP'$, $KP^{+}$ and $KP^{-}$.
Intuitively, a choice $(\IJ{i}{j},IP',AP',KP^{+},KP^{-})$ describes an element in a position that
belongs to $\IJ{i}{j}$,
that satisfies all the constraints in $IP\Meets \IJ{i}{j}$, that satisfies 
the assertions in $AP'$ and in $KP^{+}$, and does not satisfy any assertion in $KP^{-}$.
With respect to object choices, here the label is not represented by a pair of sets of assertions 
$(CP',RP')$, but just
by an interval $\IJ{i}{j}$, while the schema is a bit more complex since it has three positive components $IP'$,
$AP'$ and
$KP^{+}$, playing the roles of $CP'$ and $RP''$,
but also a negative component $KP^{-}$. 
Observe that, while $IP'$ and $AP'$ are restricted to the assertions that apply to $\IJ{i}{j}$,
we do not have this restriction for $KP$, since every counting assertion analyzes all positions of the 
array.
Hence, the schema of a choice is defined as follows.

\begin{definition}[$s(\IJ{i}{j},IP',AP',KP^{+},KP^{-})$]\label{def:schemaac}
$$
\begin{array}{lll}
\multicolumn{2}{l}{
s(\IJ{i}{j},IP',AP',KP^{+},KP^{-})
} \\[\NL]
\qquad = &(\BigAnd_{(\PreIte{l}{\RRef{x}})\in IP'} {\RRef{x}}) 
\And
(\BigAnd_{(\PostIte{i}{\RRef{x}})\in IP'} {\RRef{x}}) \\[\NL]
&\And\ 
(\BigAnd_{(\ContAfter{l}{ \RRef{x}})\in AP'} {\RRef{x}})  \\[\NL]
&\And\ 
(\BigAnd_{(\CMM{i}{j}{\RRef{x}})\in KP^{+}} {\RRef{x}})
\And
(\BigAnd_{(\CMM{i}{j}{\RRef{x}})\in KP^{-}} {\NR{x}} )
\end{array}
$$
\end{definition}

As with object groups, a generative exploration of the space of all possible solutions does not
require the generation of all possible choices, and different strategies are possible.
In our implementation, we limit ourselves to the choices where 
$KP^{-} = KP \setminus KP^{+}$, which we 
call here the co-maximal choices. 
We prove later that this strategy ensures the generativity property that we need.
More optimized strategies would be possible, but we believe that they are not 
worth the effort, since in practice the array types that we have to deal with are usually quite simple.

Hence, array {\crcombination} consists of the following steps.

\begin{compactenum}
\item compute $h = \HL(IP,AP)$;
\item for each interval $\IJ{i}{i}$ corresponding to an $i\in \IJ{1}{h}$, and for each subset $AP'$ of $AP$
and $KP'$ of $KP$
produce the corresponding co-maximal choice: %, which we indicate as $C(i,AP',KP')$:
$$%C(i,AP',KP') \ =\ 
(\IJ{i}{i},IP \Meets \IJ{i}{i},AP',KP',KP \setminus KP')
$$
and check whether the variable intersection that corresponds to the schema of that choice
is equivalent to some existing variable, and, if not, create a new variable that will become the schema
of that choice, and apply {\crcombination} to the body of this new variable, as in the case of 
object {\crcombination};
\item do the same for the interval $\IJ{h+1}{\Inf}$, and for each subset $AP'$ of $AP$
and $KP'$ of $KP$.
%,
%   obtaining the co-maximal choices that we indicate with $C(h+1,KP')$:
%   $$C(h+1,KP') \ =\ (\IJ{h+1}{\Inf},IP \Meets \IJ{h+1}{\Inf},KP',KP\Meets \IJ{h+1}{\Inf}) \setminus KP')
%$$

\end{compactenum}

As happens with object {\crcombination}, also array {\crcombination} has an exponential cost
that is quite low in practice, since in the vast majority of cases the head-length of array groups is
zero or one, and the set $AP\cup KP$ is either empty or a singleton. For this reason, we did not put any
special effort into the optimization of this phase.


\begin{property}
Array {\crcombination} can be performed in time $O(2^N)$, where $N$ is the size of the input schema.
\end{property}

%\begin{proof}
%
%\end{proof}




\subsubsection{Witness generation from a {\crcombined} array group}\label{sec:witarrj}

Array {\crcombination} applied to an array group
$\{ \ \TArr, IP, AP, KP\ \}$ with head-length $h$ produces a set of co-maximal 
choices, each characterized by an interval $\IJ{i}{j}$ with shape $\IJ{i}{i}$ when $i\leq h$, or $\IJ{h+1}{\Inf}$ otherwise, 
and by two subsets $AP', KP'$ of $AP, KP$.
We indicate with $C(i,AP',KP')$ the co-maximal choice that is characterized by these three parameters, and with
$s(i,AP',KP')$ and $s(i,AP',KP')$  its schema and the associated variable, as follows:
$$\begin{array}{llll}
\multicolumn{3}{l}{
C(i,AP',KP')\ \ \ \mbox{with\ }   1 \leq i \leq h
}\\
& \!= & \!(\IJ{i}{i},IP\Meets\IJ{i}{i},AP',KP',KP \setminus KP')  \ \ \\[\NL]
\multicolumn{3}{l}{
C(h+1,AP',KP')
}\\
& \!= & \!(\IJ{h+1}{\Inf},IP\Meets\IJ{h+1}{\Inf},AP',KP',KP \setminus KP')   \\[\NL]
\multicolumn{3}{l}{
s(i,AP',KP') \ = \ s(C(i,AP',KP'))
}\\[\NL]
\multicolumn{3}{l}{
var(i,AP',KP') \ = \ var(C(i,AP',KP'))
}
\end{array}$$


A choice $C(i,AP',KP')$ is a \emph{head choice} when $i\leq h$, and is a \emph{tail choice} when $i=h+1$. 
At any pass of the generation algorithm, a choice is \Pop\ or \Open, depending on its schema variable.

%
%Our algorithm is based on a residuation operation:
%for each assertion $\ContAfter{l}{\RRef{x}}$ in $AP$
%and $\CMM{m}{M}{\RRef{x}}$ in $KP$
% we define its residual wrt a choice $C(i,AP',KP')$
%as follows, where %$\Inf-1=\Inf$:
%$n^-$ is defined as $\Inf^-=\Inf$, $0^-=0$, $(n+1)^-=n$.
%Intuitively, $res(S,C(i,AP',KP'))$ 
%is what remains of $S$ to be satisfied after an element described by 
%$C(i,AP',KP')$ is added to the array.
%
%
%$$\begin{array}{llll}
%\begin{array}{llll}
%\mbox{if }S\notin (AP'\cup KP') : \\[\NL]
%\ \ \ (1)\ res(S,C(i,AP',KP')) = S\qquad \\[\NL]
%\mbox{if } S\in (AP'\cup KP') :\\[\NL]
%\end{array}\\[\NL]
%\ \ \ \begin{array}{llll}
%(2)\ S = \ContAfter{l}{\RRef{x}}, i\leq l: & \!\!\!\!res(S,C(i,AP',KP')) = S\qquad \\[\NL]
%(3)\ S = \ContAfter{l}{\RRef{x}}, i > l: & \!\!\!\!res(S,C(i,AP',KP')) = \True \\[\NL]
%\end{array}\\[\NL]
%\ \ \ \begin{array}{llll}
%(4)\ S = \CMM{m}{M}{\RRef{x}}, M\neq 0: & res(S,C(i,AP',KP')) = \CMM{m^-}{M^-}{\RRef{x}} \\[\NL]
%(5)\ S = \CMM{m}{M}{\RRef{x}}, M= 0: & res(S,C(i,AP',KP')) = \False \\[\NL]
%\end{array}
%\end{array}
%$$
%
%Informal explanation:
%(1): the choice is not related to the assertion $S$, hence $S$ remains to be satisfied.
%(2): the position of the choice is smaller than the index of $S$, hence $S$ remains to be satisfied.
%(3): the choice satisfies $S$.
%(4): after one element described by the choice has been inserted, we have a weaker requirement
%$ \CMM{m^-}{\Inf}{\RRef{x}}$ but a stricter constraint  $\CMM{0}{M^-}{\RRef{x}}$.
%(5): if $S$ imposes the constraint $\CMM{0}{0}{\RRef{x}}$ but $C$ includes $S$ in its $KP'$,
%then the addition of an element satisfying $C$ violates the constraint $S$.
%
%
%
%$$\begin{array}{llll}
%\begin{array}{llll}
%\mbox{if }S\notin (AP'\cup KP') : \\[\NL]
%\ \ \ (1)\ res((S,S'),C(i,AP',KP')) = S\qquad \\[\NL]
%\mbox{if } S\in (AP'\cup KP') :\\[\NL]
%\end{array}\\[\NL]
%\ \ \ \begin{array}{llll}
%(2)\ S = \ContAfter{l}{\RRef{x}}, i\leq l: & \!\!\!\!res(S,C(i,AP',KP')) = S\qquad \\[\NL]
%(3)\ S = \ContAfter{l}{\RRef{x}}, i > l: & \!\!\!\!res(S,C(i,AP',KP')) = \True \\[\NL]
%\end{array}\\[\NL]
%\ \ \ \begin{array}{llll}
%(4)\ S = \CMM{m}{M}{\RRef{x}}, M\neq 0: & res(S,C(i,AP',KP')) = \CMM{m^-}{M^-}{\RRef{x}} \\[\NL]
%(5)\ S = \CMM{m}{M}{\RRef{x}}, M= 0: & res(S,C(i,AP',KP')) = \False \\[\NL]
%\end{array}
%\end{array}
%$$
%
%
%
%We also map residuation to lists of choices $\CC$ and to sets of assertions in the natural way:
%$$\begin{array}{llllllll}
%res(S,[]) & = & S\\
%res(S,[C_1,\ldots,C_n]) & = & res(res(S,C_1),[C_2,\ldots,C_n]) \\[\NL]
%res(\Set{S_1,\ldots,S_n},\CC) & = & \Set{res(S_1,\CC),\ldots,res(S_n,\CC)} 
%\end{array}$$

Given a list of choices $\CC$ and a set of contains-after and counting assertions $\Set{AP,KP}$
(where $\Set{AP',KP'}$ abbreviates $AP'\cup KP'$),
we define the \emph{incidence} of $\CC$ over $\Set{AP,KP}$ as a function that maps each $S\in \Set{AP,KP}$
to the number of elements of $\CC$ that are guaranteed to satisfy $S$, as follows:
$$\begin{array}{llll}
\mbox{if }S\notin (AP'\cup KP') :\ & I_{C(i,AP',KP')}(S) = 0 \\[\NL]
\mbox{if }S\in (AP'\cup KP') :\ & I_{C(i,AP',KP')}(S) = 1 \\[\NL]
%\mbox{if } S\in (AP') ,\ 
%%S = \ContAfter{l}{\RRef{x}} ,\ i\leq l: & I_{C(i,AP',KP')}(S) = 0\\[\NL]
%\mbox{if } S\in (AP') ,\ 
%S = \ContAfter{l}{\RRef{x}} ,\  i > l: &   I_{C(i,AP',KP')}(S) = 1\\[\NL]
%\mbox{if } S\in (KP'): &   I_{C(i,AP',KP')}(S) = 1\\[\NL]
\multicolumn{2}{l}{
I_{[C_1,\ldots,C_n]}(S) =  \sum_{i \in \SetTo{n}} I_{C_i}(S) 
}
\end{array}
$$


We say that a list of choices $\CC$ is a solution for $\Set{AP,KP}$
when the incidence of the list satisfies all requirements and does not violate any constraint, as follows.

\begin{definition}[Well formed list, Solution] %, Minimal solution]
A list of choices for an array group is well-formed for head-length $h$ iff 
\begin{description}
\item[(1)] every choice in the 
list has either an interval $\IJ{i}{i}$ with $i\leq h$ or the interval  $\IJ{h+1}{\Inf}$; 

\item[(2)] if two consecutive choices in the list have intervals $\IJ{i}{\_}$ and $\IJ{j}{\_}$, then either
$j=i+1$ or $j=i=h+1$.
\end{description}
\end{definition}

For example, $[\,([3,3],\ldots), [4,4],\ldots), ([5,\Inf],\ldots), ([5,\Inf],\ldots)\,]$,
$[\,([5,\Inf],\ldots)\,]$, %$[\ ([2,2],\ldots)\ ]$ 
and $[\ ]$ are well formed
for head-length 4.

\begin{definition}[Solution] %, Minimal solution]
Fixed an array group
$\TG{ \ \TArr, IP, AP, KP\ }$ with head-length $h$,   a choice list  $\CC$
is a solution for the array group iff all the following hold:
\begin{compactdesc}

\item[(1)] it is well formed for $h$; 

\item[(2)] either $\CC$ is empty or the first choice has
interval $\IJ{1}{\_}$; 

\item[(3)] for every assertion $\CMM{m}{M}{x}\in KP$ we have $I_{\CC}(S) \leq M$;

\item[(4)] for every assertion $\CMM{m}{M}{x}\in KP$ we have $I_{\CC}(S) \geq m$;

\item[(5)] for every requirement $S\in AP$ we have $I_{\CC}(S) > 0$.

\end{compactdesc}

%A solution $\CC$ is \emph{minimal} if (1) no strict prefix of $\CC$ is a solution and (2) $\CC$ contains
%no tail second choice.
\end{definition}

Observe that an incidence $I_{\CC}(S)=n$ guarantees that an array described by $\CC$ 
has exactly $n$ elements that satisfy $S$ if $S\in KP$, and \emph{at least} $n$ elements that satisfy $S$ if $S\in AP$.
This happens by design, and is sufficient to guarantee the essential property that every array described by a solution is a witness
for the corresponding group.


\begin{definition}[describes-in-$\AA$]\label{def:arrdescr}
A choice $C=(\IJ{i}{j},\ldots)$ for a prepared array group
\emph{describes} \emph{in an assignment $\AA$} an element $J_l$  of an array $[\J_1,\ldots,\J_n]$, iff 
$l\in \IJ{i}{j}$ and $\J\in\AA(var(C))$.
A choice list $[C_1,\ldots,C_n]$ \emph{describes} in $\AA$  an array $\J= [\J_1,\ldots,\J_n]$ if every 
$C_l$ describes in $\AA$ the element $J_l$.
\end{definition}

\begin{property}\label{pro:solution}\label{pro:arrsolution}
For any prepared array group $$S=\TG{\TArr, IP, AP, KP}$$
with the corresponding environment $E$ and choices $\CC$, if 
$\AA$ is sound for $\E$,
if the choice list $\CC'$ over $\CC$ is a solution for $S$, and if $\J$ is described in  
$\AA$ by $\CC$,
then $\J\in\semca{S}{\E}$.
\end{property}

\begin{proof}
Consider a prepared group $S=\TG{\TArr, IP, AP, KP}$ and the corrensponding choices
$\CC$ and environment $\E$.
Let $\AA$ be sound for $\E$ and assume that $\CC'=[C_1,\ldots,C_n]$ describes $\J= [\J_1,\ldots,\J_n]$.
%Let $C_l=C(i_l,AP_i,KP_i)$.

By definition of $I_{\CC'}(S)$, for any $S=\ContAfter{i}{x}\in AP$, if $I_{\CC'}(S)=k$, then there are exactly 
$k$ choices $C$ in $\CC'$ such that $C=C(l,AP',KP')$, and $S\in AP'$.
By definition of $s(C)$ and $var(C)$, 
for all of these 
choices we have that $s(C)$ is a conjunction of $x$ with other variables,
hence $\semca{var(C)}{\E}\subseteq \semca{x}{\E}$. 
For all of these choices, the corresponding $J_l$ belongs to $\AA(var(C))$, since $\CC'$ describes in $\AA$ $J$.
Since $\AA$ is sound for $\E$, we conclude that, for these choices, we have that $J_l\in  \semca{x}{\E}$.
Hence, if $I_{\CC'}(S)>0$ with $S=\ContAfter{i}{x}$, we have at least one element of $J$ which satisfies $x$.
We must now prove that the position of that elements is greater than $i$.
By definition of choice, every choice that includes $\ContAfter{i}{x}$ has an interval that intersects $\IJ{i+1}{\Inf}$.
Since the head-length of the object group is at least $i$, every choice whose interval intersects $\IJ{i+1}{\Inf}$
is either a head-choice with interval $\IJ{j}{j}$ and $j > i$ or a tail choice with interval $\IJ{h+1}{\Inf}$ and
$h \geq i$. In both cases, every position described by that choice is strictly greater than $i$.

By definition of $I_{\CC'}(S)$, for any $S=\CMM{m}{M}{x}\in KP$, if $I_{\CC'}(S)=k$, this implies that there are exactly 
$k$ choices $C$ in $\CC'$ such that $C=C(l,AP',KP')$, and $S\in KP'$, and, as in the previous case, for all of these 
choices we have that $\semca{var(C)}{\E}\subseteq \semca{x}{\E}$. 
Since we only consider co-maximal choices, for all the other $n-k$ choices we have that $S\in KP^{-}$,
hence for the other choices we have that $s(C)$ is a conjunction of $\NR{x}$ with other varables,
hance
$\semca{var(C)}{\E}\cap \semca{x}{\E}=\emptyset$.
Since $\AA$ is sound for $\E$, and $\CC'$ describes in $\AA$ $J$, we conclude that \emph{exactly} $k$
elements of $\J$ belong to $\semca{x}{\E}$. Since $m \leq I_{\CC'}(S) \leq M$, we conclude that $\J$ satisfies
$\CMM{m}{M}{x}$.

Consider any $S=\PreIte{l}{x}\in IP$ and any choice $C$ whose interval intersects $\IJ{l}{l}$.
By construction, $\semca{var(C)}{\E}\subseteq \semca{x}{\E}$, hence, by soundness of $\AA$, the 
element described by $C$ satisfies $S$.

Consider any $S=\PostIte{i}{x}\in IP$ and any choice $C$ whose interval intersects $\IJ{i+1}{\Inf}$.
By construction, $\semca{var(C)}{\E}\subseteq \semca{x}{\E}$, hence, by soundness of $\AA$, the 
element described by $C$ satisfies $S$.

Hence, every assertion in $\TG{\TArr, IP, AP, KP}$  is satisfied by $\J$.
\end{proof}






We finally need a notion of \emph{useful choices}, which is similar in spirit to the 
\emph{R-choices} that we defined for the object case, and which will be crucial to ensure the termination
of the algorithm: a choice $C$ is \emph{useful} for a set $\Set{AP,KP}$ iff
some assertion in $\Set{AP,KP}$ is affected by $C$.
% at least one  pair $(S_o,S_r)\in\PPs$ has a non-empty intersection $S_o\cap \{AP',KP'\}$.

\begin{definition}[useful choice]
%Fixed an array group,
%\\
%$\{\ \TArr, IP, AP, KP\ \}$, with {\hel} $h$,
A choice $C(i,AP', KP')$ 
%for that group 
is \emph{useful} for a set of assertions $\Set{AP'',KP''}$ 
iff $$(\Set{AP',KP'} \cap \Set{AP'',KP''}) \neq \emptyset.$$

%If $C$ is not a first choice for $\PPs$, then it is a second choice.
\end{definition}


We can now describe our algorithm.

Our algorithm \emph{cList(hLen, aList, fLen, fInc, pChoices)} recursively solves the following generalized problem:
assume you have a list of assertions \emph{aList} and you already have a choice list \emph{firstC} of length
\emph{fLen}, whose incidence 
on  \emph{aList} is \emph{fInc};
find the rest of the list --- that is, find a well formed choice list $\CC$ such that the concatenation of \emph{firstC} with
$\CC$ is a solution for \emph{aList}.

If \emph{aList} is already satisfied by \emph{fInc}, then \emph{cList} returns the empty choice list (line 2).
Otherwise, for each $C$ in \emph{pChoices} that can describe position \emph{fLen+1}, 
we try to solve
the subproblem \emph{cList(hLen, aList, fLen+1, fInc', pChoices')}, where
\emph{fInc'} is the incidence updated after \emph{C}, and, when the position \emph{fLen+1} belongs to the tail, \emph{pChoice'}
only contains the elements of \emph{pChoice} that are still useful to solve \emph{aList} after a \emph{CLFirst}
with incidence \emph{fInc}
--- this reduction of \emph{pChoice} will be commented later on.
If such a C exists, and $\CC$ is a solution for  \emph{cList(hLen, aList, fLen+1, fInc', pChoices')}, then we return 
$[C]\mbox{++}\CC$ (lines 9-11).
If \emph{pChoices} contains no choice $C$ such that  \emph{cList(hLen, aList, fLen+1, fInc', pChoices')} has a solution,
then we return ``unsatisfiable''.

Hence, at each pass, we start from an assignment $\AA$, 
we collect all choices that are \Pop\ wrt $\AA$ in a list \emph{pChoices}, and we invoke the algorithm
 \emph{cList(\hel,0,\Set{AP,KP},allZeroes,pChoices)}.
Termination is ensured by the fact that, once we arrive to the tail, we only keep the useful choices,
hence every choice that is selected either 
(a) increments to one  the incidence over an assertion $\ContAfter{i}{\RRef{x}}$ whose incidence was zero, or
(b) increments by one the incidence over an assertion $\CMM{m}{M}{\RRef{x}}$ 
whose incidence was still below $m$,
%, or (c) residuates a $\CMM{m}{0}{\RRef{x}}$ into $\False$,
hence the algorithm stops after not more than $\key{MaxSteps}$ steps:
$$ \key{MaxSteps}\ = \ h + |AP| + \Sigma_{\CMM{m}{M}{\RRef{x}}\in KP}\ m
$$
Here, $h$ is the {\hel}, $|AP|$ is an upper bound for the (a) steps, 
and $\Sigma_{\ldots}\ m$ is an upper bound for the steps of type (b).
If the algorithm returns a solution, we use it to generate a witness by substituting
each choice with a witness from the corresponding \Pop\ schema.




\RestyleAlgo{ruled}
\begin{algorithm}
\caption{Pseudo-code for array solution generation}
\label{algo:array}
\footnotesize
%\setstretch{0.8}

\SetKw{kwIn}{in}
\SetKw{kwIsNot}{is not}
\SetKw{kwExists}{exists}
\SetKw{kwWhere}{where}
\SetKw{kwAnd}{and}

\SetKwFunction{FcList}{cList}
\SetKwFunction{FemptySat}{emptyListSatisfies}
\SetKwFunction{FtailUsefulChoices}{tailUsefulChoices}
\SetKwFunction{FpChoices}{pChoices}
\SetKwFunction{FaddChoiceToInc}{updateIncAfterChoice}
\SetKwFunction{FmaxViolated}{maxViolated}
\SetKwFunction{FinInterval}{inInterval}

\SetKwProg{Fn}{}{}{end}

\Fn{\FcList{hLen, aList, fLen, fInc, pChoices}} {
    \lIf{\FemptySat{aList, fInc}}{return [ ]}
    \If{fLen >= hLen} {
        pChoices $\gets$ \FtailUsefulChoices{pChoices, aList, fInc, hLen}\;
    }
    \For{C in \FpChoices \kwWhere \FinInterval{{hLen}+1,C}} {
        newFInc $\gets$ \FaddChoiceToInc{aList, fInc, C}\;
        \lIf{\FmaxViolated{aList, newFInc}}{continue}
        \Else{
            restSolution = \FcList{hLen, aList, fLen+1, newFInc, pChoices}\;
            \lIf{restSolution \kwIsNot null}{\Return ([C] ++ restSolution)}
            \lElse{continue}
        }
    }
    \Return null\;
}

\Fn{\FtailUsefulChoices{choices, aList, fInc, hLen}}{
%    \lIf{position $>$ limit}{\Return null}
    result = [ ]\;
    \For{C in choices \kwWhere start(C)=={hLen+1}}{
        \If{\kwExists ContAftInC \kwIn APPrimeOf(C) \\
            \kwWhere fInc(ContAftInC)=0}{add C to result\;}
        \If{\kwExists MinMaxInC \kwIn KPPrimeOf(C) \\
            \kwWhere min(MinMaxInC) $>$ fInc(MinMax)}{add C to result\;}
    }
    \Return results\;
}
\end{algorithm}



\nop{
\begin{figure}[h]
\begin{tabbing}
aa\=aa\=aa\=aa\=aa\=aaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=\kill
cList(hLen,from,r,pChoices) \+\\
  if (emptyListSatisfies(r)) return []; \\
  if (from == hLen+1) \+\\
           pChoices = tailUsefulChoices(pChoices,r,hLen); \-\\
   for C in pChoices(from) \{ \+ \\
     r = residuate(r,C);      \\
     if (False in r)  continue;  //go to next C \\
    else \{ \+ \\
       if (from <= hLen)   from = from+1; \\
       restSolution =  cList(hLen, from, r, pChoices) \\
       if (restSolution is not null) \+ \\
            return  ([C] ++ restSolution); \- \\
       else continue; // go to next C \- \\
     \} \- \\
   \} \\
return null; \- // every pChoice has been tried \\
\\


aa\=aa\=aa\=aaa\=aa\=aaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=aaaa\=\kill

// r is a list [(or,res),...,(or,res)] of original/residuated assertions \\
tailUsefulChoices(choices,r,hLen) \+\\
%  if position > limit return null; \\
  result = []; \\
  for C in choices \+ \\
  if (index(C) == hLen+1)  \+ \\
     if  (\>exists ContAft in APPrimeOf(C), (or,res) in r  \+ \\
             where or==ContAft \ )\+ \\
              add C to result; \-\- \\\
     if  (\>exists MinMax in KPPrimeOf(C), (or,res) in r  \+ \\
             where or==MinMax  and  min(res) > 0) \+ \\
              add C to result; \-\-\-\- \\\
  return(results) \- 
\end{tabbing}
\caption{Pseudo-code for array solution generation}
\label{fig:arraygeneration}
\end{figure}
}%end nop

This algorithm is sound and generative.


\begin{property}[Soundness and generativity]
The algorithm \emph{cList} is sound and generative.
\end{property}

\begin{proof}
Assume that an array group $S = \{\ \TArr, IP, AP,KP\ \}$ with {\hel} $h$ has a witness with depth
$d+1$, and consider such a witness $\J=[ \J_1, \ldots, \J_o ]$. 
For every $i$ of $\SetTo{o}$, we define 
$$\begin{array}{llll}
A(i) & = & \setst{S}{S=\ContAfter{l}{\RRef{x}},\ S\in AP,\ i > l,\ \J_i \in \semca{x}{\E}} \\[\NL]
K(i) & = & \setst{S}{S=\CMM{m}{M}{\RRef{x}},\ S\in KP,\ \J_i \in \semca{x}{\E}}
\end{array}
$$
Now we build a choice list $\CC$ that is derived from $\J$, as follows.

We define an index $i$, initialized to 1, and a \emph{cumulated incidence} function $in$, that maps every assertion to 0.
If the function $in$ satisfies already both $AP$ and $KP$, then $\CC=[]$.
Otherwise, we consider the choice $C(i,A(i),K(i))$.
We say that a choice is useful for $\Set{AP,KP}$ ``after a list of choices described by $in$'', if the choice contains
some requirements from $\Set{AP,KP}$ that are not yet satisfied by an array that is described by a list of choices 
whose incidence is $in$, which can be verified as described by function \emph{tailUsefulChoices} in the algorithm.
If $i\geq h+1$ and  $C(i,A(i),K(i))$ is not a useful choice for $\Set{AP,KP}$ after a list of choices described by $in$, then
%since by definition every element in $K(i)$ has $m=0$ in $r$, then 
we can remove $\J_i$ from
the array and what we obtain is still a witness: all requirements are already satisfied by the part of the array with
incidence $in$, and the fact that all elements after $\J_i$ decrease their position by 1 is irrelevant since we
are in the tail.
If we are not in the tail, or we are in the tail and $C(i,A(i),K(i))$ is a useful choice, 
then we leave $J_i$ in the array witness, we put $C(min(h+1,i),A(i),K(i))$ in $\CC$,
we update the cumulative incidence function $in$, we increment $i$, and we continue.

At the end of this process, we have a new witness $\J'$, obtained by deleting some elements from
the tail of $\J$, and a  choice list $\CC$ that describes $\J'$. 
By the definition of $A(i)$ and $K(i)$, every $\J'_i$ in $\J'$ belongs to $\semca{x}{\E}$ for all variables $x$ that appear positively in 
$s(C(i,AP',KP'))$ and 
does not belong to $\semca{x}{\E}$ for all variables $x$ that appear complemented in $s(C(i,AP',KP'))$,
hence it belongs to  $\semca{\NR{x}}{\E}$ for all these variables. Since $\J'$ is a witness for $S$, then
$\J'_i$ also satisfies all applicable constraints in $IP$,
hence it belongs to $\semca{s(C(i,AP',KP'))}{\E}$, hence it belongs to $\semca{var(C(i,AP',KP'))}{\E}$.
%, hence it belongs to $\semca{x(C(i,AP',KP'))}{\E}$. \GG{I must clarify the distinction
% between s(C(i,AP',KP')) and x(C(i,AP',KP'))}
If we assume that $\J$ has depth $d+1$, then every $\J'_i$ has a depth smaller than $d$, hence, for any $\AA$
that is $d$-witnessed, every variable $var(C(i,AP',KP'))$ in the list $\CC$ is populated.
Hence, the choice list $\CC$ is a list of choices that are populated, such that every tail choice $C$ is useful
after the choices that have been chosen before $C$, hence the choice list $\CC$
would be generated by our algorithm unless a different solution were generated, hence our algorithm is 
generative.

Soundness of the algorithm is immediate.
\end{proof}

\begin{property}[Complexity]
For any array group whose size is in $O(N)$, each pass of algorithm \emph{cList}
has a complexity in $O(2^{\PN})$.
\end{property}

\begin{proof}
The \emph{cList} algorithm explores at most $O(2^{\PN})$ choices at each step, and the total number of steps is at most: 
$$ \key{MaxSteps}\ = \ h + |AP| + \Sigma_{\CMM{m}{M}{\RRef{x}}\in KP}\ m
$$
By the linear constants assumption, $\key{MaxSteps}$ is in $O(N^2)$, hence the algorithm explores at most
$O({(2^{\PN})}^{N^2})=O(2^{\PN*N^2})$ tuples, and the operation that must be executed for each tuple can be performed
in time $O(2^{\PN})$.
\end{proof}
}%end iflong












%\ifshort{
%\subsection{Witness Generation from Base Types}
%
%%We have finally to specify how each typed group will generate its witnesses starting from the witnesses 
%%associated to the different variables. The treatment for these cases is dealt with in the full version \cite{long}.
%
%Witness generation for groups with a base type needs no {\crcombination}, is fully accomplished during the first
%pass, and is not difficult, as detailed below.
%}

\iflong{
\subsection{Witness Generation from Base Typed Groups}

%We have finally to specify how each typed group will generate its witnesses starting from the witnesses 
%associated to the different variables. The treatment for these cases is dealt with in the full version \cite{long}.

Witness generation for groups with a base type needs no {\crcombination}, is fully accomplished during the first
pass, and is not difficult, as detailed below.


\subsubsection{Witness generation from a canonical schema of type $\Null$ or $\Bool$}

A canonical group of type \Null\ has the shape $\{ \TNull \}$ and generates
$\xnull$.
% may only contain assertions $\Con(\Null)$,
%$\Enu(\Null)$, their negations, and $\TNull$. If one of them forbids the value $\TNull$,
%then the schema is empty, otherwise the value $\xnull$ is generated.

%Similarly for an and-merged 
A group of type $\Bool$ that does not contain any $\IBT(b)$ operator will generate either $\xtrue$ or $\xfalse$.
If it contains a collection of $\IBT(\xtrue)$ operators, it will only generate $\xtrue$, and similarly 
for $\IBT(\xfalse)$. If it contains both, it is not satisfiable, and will return ``unsatisfiable''.
%we generate the elements of $\TBool$ that are not excluded 
%by a $\Con$ assertion, an $\Enu$ assertion, or their negation.


\subsubsection{Witness generation from a canonical schema of type \Str}

A canonical group of type $\Str$ is just the conjunction of zero or more extended regular expressions,
which we reduce to one by computing their intersection, whose size is linear in the size of the input regular expressions.
At this point, we generate a witness for this regular expression, which can be done in time $O(2^\PN)$
(Section \ref{sec:regexp}).
%(using the  \emph{dk.brics.automaton}  library \cite{}.

%\begin{property}
%Witness generation for a canonical group of type $\Str$ is in $O(2^\PN)$.
%\end{property}
%
%\begin{proof}
%Not really obvious.
%\end{proof}

\subsubsection{Witness generation from a canonical schema of type \Num} %, or \TNumNotInt}



For a canonical schema of type $\Num$, we can first merge all intervals into one and
all $\Mof(m)$ operators into one, let us call it $\Mof(M)$;
if the group contains an assertion $\NotMof(n)$ with $M=n\times i$ for any integer $i$, then the group 
returns ``unsatisfiable''.
%(this are typical instances of and-merging). 
Otherwise, we obtain one interval (if none is present, we add $\Bet_{-\Inf}^{\Inf}$),
a set of zero or many $\NotMof(n)$ constraints, and one optional $\Mof(m)$
with $m\neq n\times i$ for every $i\in\IntSet$ and for every $\NotMof(n)$.
At this point, to simplify some operations, we substitute any
negative argument $n$ of $\Mof(n)$ or $\NotMof(n)$ with its opposite. 
The interval may be open at both extremes,  closed at both, or mixed. We distinguish
five cases. In the last three cases we describe an open interval $\XBet_{min}^{Max}$, but the reasoning when one extreme, or both, are included, is essentially the same.
\begin{compactenum}
\item Empty interval: we return ``unsatisfiable''.
\item One-point interval $\Bet_{m}^{m}$: if $m$ satisfies all  $\NotMof$ and  $\Mof$
     assertions we return $m$, otherwise we return ``unsatisfiable''.
\item No $\Mof(m)$, i.e.,\ many-points interval $\XBet_{min}^{Max}$ 
     with no $\Mof(m)$ constraint and $l$ $\NotMof(n_j)$ constraints: choose
      $\epsilon$ such that
      $$0 < \epsilon \leq \frac{min((Max-min),n_1,\ldots,n_l)}{l+2}$$
     If we consider the set $B = \setst{min+i\times \epsilon}{i\in \SetTo{(l+1)}}$, then 
     every value in $B$ satisfies $\XBet_{min}^{Max}$, and no assertion $\NotMof(n_j)$
     can be violated by two distinct values in $B$, hence at least one value in $B$ is a witness.
\item Finite $Max-min$ and $\Mof$, i.e.,\ interval $\XBet_{min}^{Max}$ with a $\Mof(m)$ constraint 
   and finite values for both $min$ and $Max$: we list 
   all multiples of $m$ starting from $min$ (excluded in case of $\XBet$) until we find one 
   that satisfies all $\NotMof$ assertions, or until we go over $Max$ (excluded or included depending on the interval), in which case we return ``unsatisfiable''.
\item Infinite $Max-min$ and $\Mof$, i.e.,\ interval $\XBet_{min}^{Max}$ where either $min$ or
   $Max$ is not finite, and with a $\Mof(m)$ constraint: 
   bring all arguments of $\Mof(m)$ and $\NotMof(n)$ into a fractional form where they share the same
   denominator $d$, as in $\Mof(M/d)$, $\NotMof(n_j/d)$. Select any prime number $p$ that is strictly 
   bigger than every $n_j$ and such that either $p\times M/d$ or its
   opposite belongs to the interval. Such a number clearly exists, and
   it is easy to prove that primality of $p$ and the fact that $(M/d)\neq (n_j/d)\times i$ for every $i\in\IntSet$ 
   and for every $\NotMof(n_j/d)$, imply that $p\times M/d$ satisfies all $\NotMof$ assertions.
 \end{compactenum}

\begin{property}
If a group of type $\Num$ has a witness, then the above algorithm will return a witness.
\end{property}

\begin{proof}
The only difficult case is case (5).
  Assume, towards a contradiction, that exists $n_j/d$ and an integer $i$ with 
  $p\times M/d = i\times (n_j/d) $, that is $p\times M = i\times n_j$.
Since $p$ is prime and is bigger than $n_j$, then $p$ is prime wrt $n_j$.
Since $p$ is a factor of $i\times n_j$ and is prime wrt $n_j$,
then $p$ is a factor of $i$,
hence there exists an integer $i'$ such that $i=i'\times p$,
that is,
$p\times M = i'\times p \times n_j$,
that is, $M = i' \times n_j$, which is impossible.
\end{proof}

\begin{property}
If a group of type $\Num$ has a witness, one can be generated in time $O(2^{\PN})$,
where $N$ is the size of the input schema.
If a group of type $\Num$ has a witness, this fact can be proved in time $O(2^{\PN})$.
\end{property}

\begin{proof}
Here we do not need the linear constant assumption over any of the involved parameters.
Let $N$ be the size of the input schema.
In case (3), we try $O(N)$ witnesses.
In case (4), we must try at most $(Max-min)/m$ possible witnesses, which is in $O(2^N)$, because of
binary notation.
In case (5), we exploit the fact that the numbers are decimal, hence the number of digits of $d$ is 
linear in $N$, hence the size of every $n_j$ is still limited by $N$. 
We must also assure that either $p\times M/d$ or its opposite belongs to the interval.
For example, when $min$ is finite, $p$ must satisfy 
$(p\times M)/d > min$ hence  $p > min\times d / M$, and again
all the constants have a bitmap representation linear in $N$. 
A prime number greater than $k$ can be generated in time
that is polynomial in $k$, hence we are still in $O(2^{\PN})$.
\end{proof}
%\DC{again, we should for numbers precise how density is ensured ....}
}%end iflong


\ifshort{
\bcolormeta
\subsection{Completeness and correctness}

\mrevmeta{The algorithm that we describe in this paper is correct and complete.}{M.3}

\begin{theorem}[Correctness and completeness]
The algorithm described in this paper is correct and complete: it returns a witness if, and only if,
the schema admits a witness, and otherwise it indicates that the schema is not satisfiable
\end{theorem}

\begin{proof}
The phases described in Section \ref{sec:firstphases} transform the given schema into an equivalent one,
by Property \ref{pro:preliminarycc}.
By Property \ref{pro:coandco},
the bottom-up algorithm described in Section \ref{sec:bottomup} terminates with success if, and only if
the schema admits a witness, and otherwise indicates that the schema is not satisfiable,
provided that the algorithm used for preparation and generation is sound and generative.
The algorithm that we use for preparation and generation of objects is sound and generative
by Theorem \ref{the:sogen}.
The proof that the algorithm that we use for preparation and generation of arrays is sound and generative
can be found in the full paper \cite{attouche2022witness}.
\end{proof}

\ecolormeta
}



